Preservation of shadowing in discrete dynamical systems

We look at the preservation of various notions of shadowing in discrete dynamical systems under inverse limits, products, factor maps and the induced maps for symmetric products and hyperspaces. The shadowing properties we consider are the following: shadowing, h-shadowing, eventual shadowing, orbital shadowing, strong orbital shadowing, the first and second weak shadowing properties, limit shadowing, s-limit shadowing, orbital limit shadowing and inverse shadowing.

==> Graveyard.tex <==
%% h-shadowing and factor maps (continuity lemma issue). Certainly h-shadowing is preserved by conjugacy.

\subsection{Factor maps}
\begin{lemma}
\label{pullbacklemma}
Suppose $X$ and $Y$ are Tychonoff spaces (i.e. $T_{3\frac{1}{2}}$) with $X$ compact and $\varphi\colon X\to Y$ continuous. Let $\mathscr{U}_Y$ be a compatible uniformity for $Y$ and $\mathscr{U}_X$ the uniformity associated with $X$. Then, for all $E\in \mathscr{U}_X$, there exists $D \in \mathscr{U}_Y$ such that for all $y\in Y$, if $x\in\varphi^{-1}(B_D(y))$ then there exists $x'\in\varphi^{-1}(y)$ with $(x,x')\in E$.
\end{lemma}
\begin{proof}
Suppose the lemma is false. Then, there exists some symmetric $E\in \mathscr{U}_X$ such that for all $D\in \mathscr{U}_Y$, there exists $y \in Y$ and there exists $x_D\in\varphi^{-1}(B_D(y))$ such that for all $x'\in\varphi^{-1}(y)$ one has $(x_D,x')\notin E$. Notice that $(x_D)_{D\in \mathscr{U}_Y}$ forms a net (where $D_1 \geq D_2$ iff $D_1 \subseteq D_2$). By compactness there is a subnet which converges to a point $z \in X$. Clearly  $\varphi(x_D)_{D \in \mathscr{U}_Y}\to y$. By continuity of $\varphi$, one then has $y=\varphi(z)$, resulting in $z\in\varphi^{-1}(y)$ providing the required contradiction.
\end{proof}


\begin{theorem}\label{ThmALPhshad}
Suppose that $\varphi \colon (X,f)\to (Y,g)$ is a factor map.
\begin{enumerate}
	\item If $(X,f)$ has h-shadowing and $\varphi$ almost lifts pseudo-orbits, then $(Y,g)$ has h-shadowing.
	\item If $(Y,g)$ has h-shadowing, then $\varphi$ almost lifts pseudo orbits.
\end{enumerate}
\end{theorem}
\begin{proof}
\begin{enumerate}
\item Fix $E \in \mathscr{U}_Y$. Let $E_0\in\mathscr{U}_Y$ be such that $2E_0 \subseteq E$. By compactness of $X$ and continuity of $\varphi$, there exists $D_1 \in \mathscr{U}_X$ such that for all $x,x'\in X$ with $(x,x')\in D_1$ one has $(\varphi(x),\varphi(x'))\in E_0$. Furthermore, let $D_2 \in \mathscr{U}_X$ be such that every $D_2$-pseudo-orbit is $D_1$-h-shadowed. Let $D_3 \in \mathscr{U}_X$ be such that $2D_3 \subseteq D_2$. %Let $V_0\in \mathscr{U}_Y$ be such that $\phi^{-1}(2V_0) \subseteq D_2$. 
One may then use Lemma \ref{pullbacklemma} with $\varphi$ and $D_3$ to deduce the existence of a $V_0 \in \mathscr{U}_Y$ such that if $x\in \varphi^{-1}(B_{V_0}(y))$ for some $y\in Y$, then there exists $x'\in\varphi^{-1}(y)$ such that $(x,x')\in D_3$. Finally, using the almost lifting pseudo-orbit condition with $V:=E_0\cap V_0$ and $D_3$ one obtains a $W \in \mathscr{U}_Y$ such that if $(y_i)_{i\geq 0}\subseteq Y$ is an $W$-pseudo-orbit, then there exists a $D_3$-pseudo-orbit $(x_i)_{i\geq 0}\subseteq X$ with $(\varphi(x_i),y_i)\in V$ for each $i\geq 0$. \par
Now, suppose that $(y_i)_{i\leq n}\subseteq Y$ is a finite $W$-pseudo-orbit. Extend this to a $W$-pseudo-orbit by $y_{j+n}=f^j(y_n)$ for $j\geq 1$. Using the above, one obtains a $D_3$-pseudo-orbit $(x_i)_{i\geq 0}$ in $(X,f)$ with $(\varphi(x_i),y_i) \in V$ for all $i\geq 0$.  In particular, one has $x_n\in\varphi^{-1}(B_{V_0}(y_n))$, and so there exists some $x\in \varphi^{-1}(y_n)$ whereby $(x,x_n)\in D_3$. Observe now that $\{x_0,x_1,\ldots,x_{n-1},x\}$ is a finite $D_2$-pseudo-orbit in $X$; indeed, $(f(x_i),x_{i+1})\in D_3$ for $i\leq n-2$ and since $(f(x_{n-1}),x_n),(x_n,x)\in D_3$ by definition
	\begin{align*}
		(f(x_{n-1}),x)\in 2D_3 \subseteq D_2.
	\end{align*}
Let $z\in X$ $D_1$-h-shadow this finite orbit; we then claim that $\varphi(z)$ $E$-h-shadows $(y_i)_{i\leq n}$. Indeed, for $i<n$, $(g^i(\varphi(z)),y_i)=(\varphi(f^i(z)),y_i)$. Since, for any $i<n$, $(\varphi(f^i(z)),\varphi(x_i)),(\varphi(x_i),y_i) \in E_0$ it follows that  $(\varphi(f^i(z)),y_i) \in 2E_0 \subseteq E$. But $(g^i(\varphi(z)),y_i)=(\varphi(f^i(z)),y_i)$ for any $i<n$. Hence $(g^i(\varphi(z)),y_i) \in E$ for all $i<n$. Finally, since $f^n(z)=x\in\varphi^{-1}(y_n)$ one has $\varphi(f^n(z))=g^n(\varphi(z))=y_n$. Thus, every $W$-pseudo-orbit of $(Y,g)$ is $E$-h-shadowed.
\item Observe that since $(Y,g)$ has h-shadowing then it also has shadowing and so $\varphi$ is ALP by Theorem \ref{ShadowALP}.
\end{enumerate}
\end{proof}


%% Inverse shadowing and factor maps. Again, certainly preserved by topological conjugacy.

\subsection{Factor maps}


\begin{theorem}
Suppose that $(X,f)$ and $(Y,g)$ are dynamical systems of compact Hausdorff spaces. If $(X,f)$ has $\mathcal{T}_0$-inverse shadowing and $\varphi \colon (X,f)\to (Y,g)$ is a factor map, then $(Y,g)$ has $\mathcal{T}_0$-inverse shadowing.
\end{theorem}
\begin{proof}
Fix $E \in \mathscr{U}_Y$. Extract $D_1 \in \mathscr{U}_X$ from the uniform continuity of $\varphi$ due to the compactness of $X$ so that if $x,x'\in X$ with $(x,x')\in D_1$, then $(\varphi(x),\varphi(x'))\in E$. Next, suppose that $D_2 \in \mathscr{U}_X$ is extracted from the definition of $D_1$ positive $\mathcal{T}_0$-inverse shadowing for $X$. Lastly, suppose that $W \in \mathscr{U}_Y$ corresponds to $D_2$ in Lemma \ref{pullbacklemma}. That is, for all $y\in Y$, if $x\in\varphi^{-1}(B_{W}(y))$, then there exists $x'\in\varphi^{-1}(y)$ with $(x,x')\in D_2$.
\par Now, consider a $W$-method $\psi\in\mathcal{T}_0(g,W)$; we construct a $D_2$-method $\hat{\psi}\in\mathcal{T}_0(f,D_2)$ that lifts to $\psi$. Consider $z\in X$ and then consider the $D_2$-pseudo orbit $\psi(\varphi(z))$. Define $z_0:=z$ and observe that by definition,
	\begin{align*}
		(g(\psi(\varphi(z))_0),\psi(\varphi(z))_1)\in W.
	\end{align*}
This means that 	
	\begin{align*}
		g(\varphi(z_0))=\varphi(f(z_0))\in B_{W}(\psi(\varphi(z))_1),
	\end{align*}
	so that
	\begin{align*}
		f(z_0)\in\varphi^{-1}(B_{W}(\psi(\varphi(z))_1)),
	\end{align*}
	and hence there exists $z_1\in\varphi^{-1}(\psi(\varphi(z))_1)$ such that
	\begin{align*}
		(f(z_0),z_1) \in D_2.
	\end{align*}
Suppose that $z_0,\ldots, z_{k-1}\in X$ have been defined so that
	\begin{enumerate}
		\item $z_0:= z$,
		\item $z_i\in\varphi^{-1}(\psi(\varphi(z))_i)$ for all $i=1,\ldots, k-1$,
		\item $(f(z_i),z_{i+1}) \in D_2$ for all $i=0,\ldots,k-2$.
	\end{enumerate}
To construct $z_k$, observe that
	\begin{align*}
		\varphi(f(z_{k-1}))=g(\varphi(z_{k-1}))=g(\psi(\varphi(z))_{k-1}),
	\end{align*}
and by definition,
	\begin{align*}
		(g(\psi(\varphi(z))_{k-1}),\psi(\varphi(z))_k)\in W,
	\end{align*}
so that 
	\begin{align*}
		f(z_{k-1})\in\varphi^{-1}(B_{W}(\psi(\varphi(z))_k)).
	\end{align*}
Thus, there exists
	\begin{align*}
		z_{k}\in\varphi^{-1}(\psi(\varphi(z))_{k})
	\end{align*}
such that
	\begin{align*}
		(f(z_{k-1}),z_k)\in D_2,
	\end{align*}
as required. Recursively, this defines a positive $D_2$-pseudo-orbit $(z_k)_{k\geq 0}$ originating from $z_0=z$ and such that $(\varphi(z_k))_{k\geq 0}=(\psi(\varphi(z))_k)_{k\geq 0}$. Thus, if one defines $\hat{\psi}(z)=(z_k)_{k\geq 0}$ one has $\hat{\psi}\in\mathcal{T}_0(f,D_2)$ and,
	\begin{align*}
		\varphi(\hat{\psi}(z)_k)=\psi(\varphi(z))_k.
	\end{align*}
So, consider $y\in Y$ and let $\psi\in\mathcal{T}_0(g,W)$. Then, one can construct a lifting method $\hat{\psi}\in\mathcal{T}_0(f,D_2)$ as above. Take $x\in\varphi^{-1}(y)$ and utilise the positive $\mathcal{T}_0$-inverse shadowing in $(X,f)$ to extract $x'\in X$ such that 
	\begin{align*}
		(f^k(x),\hat{\psi}(x')_k) \in D_1
	\end{align*}
for all $k\geq 0$. Thus, by the uniform continuity condition, one obtains
	\begin{align*}
		(\varphi(f^k(x)),\varphi(\hat{\psi}(x')_k))=(g^k(y),\psi(\varphi(x'))_k) \in E
	\end{align*}
for all $k\geq 0$ as required.

\end{proof}


==> Preliminaries/ALP_Definitions.tex <==
\section{Maps which almost lift pseudo orbits}

\begin{definition} Suppose $X$ and $Y$ are compact Hausdorff spaces, $f\colon X \to X$ and $g \colon Y \to Y$ are continuous. A factor map $\varphi \colon (X,f) \to (Y,g)$ \textit{almost lifts pseudo-orbits (ALP)} if for every $V \in \mathscr{U}_Y$ and every $D \in \mathscr{U}_X$ there exists $W \in \mathscr{U}_Y$ such that for every $W$-pseudo-orbit $(y_i)_{i \in \omega}$ in $Y$, there exists a $D$-pseudo-orbit $(x_i)_{i \in \omega}$ in $X$ such that $(\varphi(x_i),y_i) \in V$ for all $i \in \omega$. 
\end{definition}

\begin{definition}
A surjective semiconjugacy $\varphi \colon X\to Y$ between compact Hausdorff spaces $X$ and $Y$ \textit{eventually almost lifts pseudo orbits (eALP)} if for every $E \in \mathscr{U}_Y$ and $D \in \mathscr{U}_X$ there is $V \in \mathscr{U}_Y$ such that for every $V$-pseudo-orbit $(y_i)$ in $Y$ is a $D$-pseudo-orbit $(x_i)$ in $X$ such that $(\phi(x_i))_{i \in \omega}$ eventually-$E$-shadows $(y_i)_{i \in \omega}$..
\end{definition}

\begin{definition}
A surjective semiconjugacy $\varphi \colon X\to Y$ is \emph{oALP} if for every $V \in \mathscr{U}_Y$ and $D \in \mathscr{U}_X$ there exists $W \in \mathscr{U}_Y$ such that for all $W$-pseudo-orbits $(y_i)\subseteq Y$, there exists a $D$-pseudo-orbit $(x_i)\subseteq X$ for which 
	\begin{align*}
    	(\varphi(\overline{\{x_i\}_{i\in\omega}}),\overline{\{y_i\}_{i\in\omega}}) \in 2^V.
     \end{align*}
\end{definition}

\begin{definition}
A surjective semiconjugacy $\varphi \colon X\to Y$ between compact Hausdorff spaces $X$ and $Y$ is \emph{w1ALP} if for every $V \in \mathscr{U}_Y$ and $D \in \mathscr{U}_X$ there exists $W \in \mathscr{U}_Y$ such that for all $W$-pseudo-orbits $(y_i)\subseteq Y$, there exists a $D$-pseudo-orbit $(x_i)\subseteq X$ for which $\{y_i\})_{i \in \omega} \subseteq B_{E}(\{\varphi(x_i)\}_{i \in \omega})$.
\end{definition}



==> Preliminaries/Summary.tex <==

\section{Summary of Results}\label{SectionSummary}

\begin{tabular}{c||c|c|c|c|c|}
 & $2^X$ & $F_n(X)$ & $\pi$ & $\varprojlim$ & $\prod$  \\
\hline
\hline
shadowing&\y&\x \, (but \y for $F_2(X)$) & iff ALP &\y&\y\\
\hline

h-shadowing&\y&\x \, (but \y for $F_2(X)$)&iff ALP&\y&\y\\
\hline
eventual shadowing&\x&\x \, (but \y for $F_2(X)$)&iff eALP&\y&\y\\
\hline
orbital shadowing&\x&\x& iff oALP &\y&\x\\
\hline
strong orbital shadowing&\x&\x& iff soALP &\y&\x\\
\hline
weak 1 shadowing&\x&\x& iff w1ALP &\y&\x\\
\hline
weak 2 shadowing&\y&\y&\y&\y&\y\\
\hline
limit shadowing &?&?&iff ALAP&$\sigma$&\y\\
\hline
s-limit shadowing&?&?&iff ALA$\epsilon$P &$\sigma$&\y\\
\hline
asymptotic orbital shadowing&?&?& iff oALAP &?&?\\
\hline
orbital limit shadowing&?&?& iff oALAP&?&?\\
\hline
%orbital limit shadowing&&&&&&&&\\
%\hline
%orbital limit shadowing&&&&&&&&\\
%\hline
%orbital limit shadowing&&&&&&&&\\
%\hline
%orbital limit shadowing&&&&&&&&\\
%\hline
%orbital limit shadowing&&&&&&&&\\
%\hline
%orbital limit shadowing&&&&&&&&\\
%\hline
unique shadowing&?&\x&only if ALP&?&?\\
\hline
Lipschitz shadowing&\y&?&?&?&?\\
\hline
Inverse shadowing&\y&?&any onto semiconj.&\y&\y\\


\end{tabular}

==> Sections/LimitShadowingProperties.tex <==
\section{Limit shadowing properties and semi-conjugacies}

`ALP' type definitions are precisely what are needed to ensure various limit shadowing properties are preserved under semi-conjugacy. Whilst we list the results here, we omit their proofs - noting the similarity they hold to those of theorems \ref{ThmALPhshad}, \ref{ThmALPeventualShad}, \ref{ThmALPOrbShad}, \ref{ThmALPFirstWeakShad} and \ref{ThmALPStrongOrbShad}.

\begin{definition}
A surjective semiconjugacy $\varphi \colon X\to Y$ is \emph{oALAP} if for every asymptotic pseudo-orbit $(y_i)_{i \in \omega}\subseteq Y$, there exists an asymptotic-pseudo-orbit $(x_i)_{i \in \omega}\subseteq X$ such that for any $E \in \mathscr{U}_Y$ there exists $N \in \mathbb{N}$ such that for all $i \geq N$
	\begin{align*}
    	(\varphi(\overline{\{x_i\}_{i\in\omega}}),\overline{\{y_i\}_{i\in\omega}}) \in E.
     \end{align*}
\end{definition}


\begin{theorem}\label{ThmALPasympOrbLimShad}
Suppose that $\varphi \colon (X,f)\to (Y,g)$ is a surjective semiconjugacy.
	\begin{enumerate}
		\item If $(X,f)$ exhibits asymptotic orbital limit shadowing and $\varphi$ is oALAP, then $(Y,g)$ exhibits orbital shadowing.
		\item If $(Y,g)$ exhibits asymptotic orbital limit shadowing, then $\varphi$ is oALAP.
	\end{enumerate}
\end{theorem}


In \cite{GoodMeddaugh2016} the authors prove the following theorem.

\begin{theorem}\textup{\cite[Theorem 22]{GoodMeddaugh2016}} Let $(X,f)$ be a dynamical system where $X$ is a compact metric space. Then the following are equivalent:
\begin{enumerate}
    \item $f$ has the asymptotic orbital shadowing property;
    \item $f$ has the asymptotic strong orbital shadowing property;
    \item $f$ has the orbital limit shadowing property; and
    \item $\omega_f =ICT(f)$.
\end{enumerate}
\end{theorem}
Where $\omega_f$ is the collection of all $\omega$-limit sets of $f$, whilst $ICT(f)$ is the collection of all \textit{internally chain transitive} sets; a closed set $A \subseteq X$ is internally chain transitive provided for any pair $x,y \in A$ and any $\epsilon>0$ there exists a sequence $x=x_0, x_1, \ldots, x_n=y$ for which $d(f(x_i),x_{i+1}) < \epsilon$ for all $i \in \{0,\ldots, n-1\}$. Combining this with our Theorem \ref{ThmALPasympOrbLimShad} gives that oALAP is precisely the property needed to preserve, under semi-conjugacy, the property of $\omega(f)=ICT(f)$.

\begin{corollary}
Suppose that $\varphi \colon (X,f)\to (Y,g)$ is a surjective semiconjugacy between compact metric spaces $X$ and $Y$.
\begin{enumerate}
    	\item If $\varphi \colon X\to Y$ oALAP and $\omega(f)=ICT(f)$, then $\omega(g)=ICT(g)$. 
        \item If $\omega(g)=ICT(g)$, then $\varphi$ is oALAP.
    \end{enumerate}
\end{corollary}

\subsection{Tychonoff product}


\begin{theorem}
Let $\Lambda$ be an arbitrary indexation set and, for each $\lambda \in \Lambda$, let $(X_\lambda, f_\lambda)$ be a compact Hausdorff system with limit shadowing. Then the product system $(X,f)$, where $X=\prod_{\lambda \in \Lambda} X_\lambda$, has limit shadowing.
\end{theorem}

\begin{proof}
Let $(x_i)_{i \in \omega}$ be an asymptotic pseudo orbit in $X$. Then, for any $\lambda \in \Lambda$, $\left(\pi_\lambda(x_i)\right)_{i \in \omega}$ is an asymptotic pseudo orbit in $X_\lambda$. By limit shadowing in these component spaces, for each $\lambda$ there exists $y_\lambda \in X_\lambda$ which limit shadows $\left(\pi_\lambda(x_i)\right)_{i \in \omega}$. Let $y \in X$ be such that $\pi_\lambda(y)=y_\lambda$ for any $\lambda \in \Lambda$. We claim $y$ limit shadows $(x_i)_{i \in \omega}$. 

Let $E \in \mathscr{U}$ be given; this entourage is refined by one of the form
\[ \prod _{\lambda \in \Lambda} E_\lambda,\]
where $E_\lambda \in \mathscr{U}_\lambda$ for all $\lambda \in \Lambda$ and $E_\lambda =X_\lambda \times X_\lambda$ for all but finitely many of the $\lambda$'s. Let $\lambda_j$, for $1\leq j \leq k$, be precisely those elements in $\Lambda$ for which $E_\lambda  \neq X_\lambda \times X_\lambda$ (if there are no such elements then we are done). For each such $j$, let $M_j \in \mathbb{N}$ be such that for any $n \geq M_j$ $(f^n(y_{\lambda_j}) \pi_{\lambda_j}(x_n)) \in E_{\lambda_j}$. Take $M \coloneqq \max_{1 \leq j \leq k} M_j$. It follows that, for any $n \geq M$, $(f^n(y),x_n) \in E$.
\end{proof}

\begin{theorem}
Let $\Lambda$ be an arbitrary indexation set and, for each $\lambda \in \Lambda$, let $(X_\lambda, f_\lambda)$ be a compact Hausdorff system with s-limit shadowing. Then the product system $(X,f)$, where $X=\prod_{\lambda \in \Lambda} X_\lambda$, has s-limit shadowing.
\end{theorem}

\begin{proof}
We start by checking condition (2) in the definition of s-limit shadowing.
Let $E \in \mathscr{U}$ be given; this entourage is refined by one of the form
\[ \prod _{\lambda \in \Lambda} E_\lambda,\]
where $E_\lambda \in \mathscr{U}_\lambda$ for all $\lambda \in \Lambda$ and $E_\lambda =X_\lambda \times X_\lambda$ for all but finitely many of the $\lambda$'s. Let $\lambda_j$, for $1\leq j \leq k$, be precisely those elements in $\Lambda$ for which $E_\lambda  \neq X_\lambda \times X_\lambda$ (if there are no such elements then we are done).

By s-limit shadowing in each component space, there exist entourages $D_{\lambda_i} \in \mathscr{U}_{\lambda_i}$ such that every asymptotic $D_{\lambda_i}$-pseudo-orbit is asymptotically $E_{\lambda_i}$-shadowed. Note that, for every $\lambda \in \Lambda \setminus\{\lambda_i \mid 1 \leq i \leq k\}$ every asymptotic pseudo-orbit is asymptotically $E_{\lambda}$-shadowed. For $\lambda \in \Lambda \setminus\{\lambda_i \mid 1 \leq i \leq k\}$ take $D_\lambda=X \times X$.
Let
\[ D \coloneqq \prod _{\lambda \in \Lambda} D_\lambda.\]

Now let $(x_j)_{j \in \omega}$ be an asymptotic $D$-pseudo-orbit. Then $(\pi_{\lambda_i}(x_j))_{j \in \omega}$ is a $D_{\lambda_i}$-pseudo-orbit in $X_{\lambda_i}$, which is asymptotically $E_{\lambda_i}$-shadowed by a point $z_i \in X_{\lambda_i}$. Furthermore $(\pi_{\lambda}(x_j))_{j \in \omega}$ is an asymptotic pseudo-orbit in $X_\lambda$ which is asymptotically shadowed by a point $z_\lambda$. Let $z \in X$ be such that $\pi_\lambda(z)=z_\lambda$ for all $\lambda \in \Lambda \setminus\{\lambda_i \mid 1 \leq i \leq k\}$ and $\pi_{\lambda_i}(z)=z_{\lambda_i}$ for each $i$. It is easy to see that $z$ asymptotically $E$-shadows  $(x_j)_{j \in \omega}$.

The result follows by Theorem \ref{ThmProductPreserveShadowing}.
\end{proof}
